Fair Adversarial Gradient Tree Boosting

Fair classification has become an important topic in machine learning research. While most bias mitigation strategies focus on neural networks, we noticed a lack of work on fair classifiers based on decision trees even though they have proven very efficient. In an up-to-date comparison of state-of-the-art classification algorithms in tabular data, tree boosting outperforms deep learning. For this reason, we have developed a novel approach of adversarial gradient tree boosting. The objective of the algorithm is to predict the output $Y$ with gradient tree boosting while minimizing the ability of an adversarial neural network to predict the sensitive attribute $S$. The approach incorporates at each iteration the gradient of the neural network directly in the gradient tree boosting. We empirically assess our approach on 4 popular data sets and compare against state-of-the-art algorithms. The results show that our algorithm achieves a higher accuracy while obtaining the same level of fairness, as measured using a set of different common fairness definitions.

==> trash.tex <==
\begin{comment}
\subsection{Demographic Parity as Fairness Metric}
To achieve demographic parity as defined in Section~\ref{sec:demographic_parity}, we exclusively provide the current prediction $\widehat{Y}$ to the adversary $A$ at each iteration of the GTB. This means that the adversarial network only has the $m$-th prediction to reconstruct the sensitive feature, and also that the desired output is known to us at each step. Thus, using backpropagation, we can penalize the gradient of the GTB in order to lose the information required to reconstruct the sensitive attribute. This approach implies to minimize the positive rate difference between the two different values of the sensitive class at each iteration.


The predictor and the adversarial classifier are trained simultaneously to minimize the value function $V$ which represents the total negative log-likelihood: 

\begin{eqnarray}
    V(f,\theta_{A}) 
    = \mathcal{L}_f(Y,f(X))-\lambda\mathcal{L}_{\theta_{A}}(S,A_{\theta_{A}}(f(X)))
    \label{valuefunction}
\end{eqnarray}

where $\mathcal{L}_f$ and $\mathcal{L}_{\theta_{A}}$ are the negative log-likelihood of $f$ and $A$, respectively:

\begin{eqnarray}
    \begin{aligned}
    \mathcal{L}_f(Y,f(X)) &= -\sum_{i=1}^{n}\log p_{f}(y_i|x_i)\\
    \mathcal{L}_{\theta_{A}}(S,A_{\theta_{A}}(f(X))) &= -\sum_{i=1}^{n}\log p_{\theta_{A}}(s_i|f(x_i))
    \end{aligned}
\end{eqnarray}
    
    
    
        
    

%\max\limits_F \min\limts_A \sum_{i=1}^{n}\log p_{F}(y_i|x_i) - \sum_{i=1}^{n}\log (p_{{A}}(s_i|F(x_i))) \\

%   \max\limits_F \min\limts_A \sum_{i=1}^{n}\log p_{F}(y_i|x_i) - \sum_{i=1}^{n} \sum_{\hat{y} \in \{0,1\}} p_{F}(\hat{y}|x_i) \log (p_{A}(s_i|\hat{y})) \\  

%p_{{A}}(s=1|\hat{y}=1)=\frac{\sum_{i,s_i=1}F(x_i)}{\sum_{i}F(x_i)} \\
%p_{{A}}(s=1|\hat{y}=0)=\frac{\sum_{i,s_i=1}(1-F(x_i))}{\sum_{i}(1-F(x_i))} 
    
where $\forall x_i \in X,\forall y_i \in Y,\forall s_i \in S$. The tuneable hyperparameter $\lambda$ controls the impact of the adversarial network. In order to find the fairest GTB $\widehat{f}$ and the optimal parameters of the adversary, $\widehat{\theta}_{A}$, we optimize the model by finding the min-max solution:
    \begin{flalign}
    \widehat{f},\widehat{\theta}_{A} =\operatorname*{arg}\operatorname*{min}_f\operatorname*{max}_{\theta_{A}} V(f,\theta_{A})
    \end{flalign}

\subsection{Equalized Odds as Fairness Metric}
Optimizing for equalized odds as described in Section~\ref{sec:equalized_odds} we provide the current prediction $\widehat{Y}$ along with the ground truth label $Y$ to the adversarial neural network at each iteration. By adding $Y$, we preserve the information when $Y$ really is equal to 1 which implies to minimize at each iteration the difference between the True Positive Rate (TPR) and True Negative Rate (TNR) for the two different values of the sensitive class. %Let's take the example of an adversary with a simple logistical regression. By only providing y and yhat, the weighting assigned to y allows to modify by translating the treshold
%prediction of the adversary is modify for y is true or false by translating the threshold using the .

As for the previous metric, the predictor and the adversarial classifier are trained simultaneously to minimize the total negative log-likelihood: 
    \begin{eqnarray}
    V(f,\theta_{A}) 
    = \mathcal{L}_f(y,f(X))-\lambda\mathcal{L}_{\theta_{A}}(s,A_{\theta_{A}}(f(X),y))
    \end{eqnarray}

where $\mathcal{L}_f$ and $\mathcal{L}_{\theta_{A}}$ are the negative log-likelihood of $f$ and $A$, respectively:
    \begin{eqnarray}
    \begin{aligned}
    \mathcal{L}_f(Y,f(X)) &= -\sum_{i=1}^{n}\log p_{f}(y_i|x_i)\\
    \mathcal{L}_{\theta_{A}}(S,A_{\theta_{A}}(f(X),y)) &= -\sum_{i=1}^{n}\log p_{\theta_{A}}(s_i|f(x_i),y)
    \end{aligned}
    \end{eqnarray}

We optimize the model by finding the min-max solution as follows:
    \begin{flalign}
    \widehat{f},\widehat{\theta}_{A} =\operatorname*{arg}\operatorname*{min}_f\operatorname*{max}_{\theta_{A}} V(f,\theta_{A})
    \end{flalign}

\end{comment}   
